Hierarchical State Machines as Modular Horn Clauses

In model based development, embedded systems are modeled using a mix of dataflow formalism, that capture the flow of computation, and hierarchical state machines, that capture the modal behavior of the system. For safety analysis, existing approaches rely on a compilation scheme that transform the original model (dataflow and state machines) into a pure dataflow formalism. Such compilation often result in loss of important structural information that capture the modal behaviour of the system. In previous work we have developed a compilation technique from a dataflow formalism into modular Horn clauses. In this paper, we present a novel technique that faithfully compile hierarchical state machines into modular Horn clauses. Our compilation technique preserves the structural and modal behavior of the system, making the safety analysis of such models more tractable.

==> eptcsdata.tex <==
\providecommand{\firstpage}{15}
\providecommand{\publicationstatus}{J. P. Gallagher and P. R\"ummer (Eds.): 3rd Workshop\\
on Horn Clauses for Verification and Synthesis (HCVS)\\
EPTCS 219, 2016, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.219.2}{10.4204/EPTCS.219.2}}
\pdfoutput=1


==> tikzlibraryshadows.blur.code.tex <==
%%
%% This is file `tikzlibraryshadows.blur.code.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% pgf-blur.dtx  (with options: `texfile')
%% Copyright 2012 Martin Giese, martingi@ifi.uio.no
%% 
%% This file is under the LaTeX Project Public License
%% See CTAN archives in directory macros/latex/base/lppl.txt.
%% 
%% DESCRIPTION:
%%   `pgf-blur' adds blurred/faded/fuzzy shadows to TikZ/PGF
%% 


\def\fileversion{1.01}
\def\filedate{2012/04/24}
\message{ v\fileversion, \filedate}
\usetikzlibrary{shadows}
\usetikzlibrary{calc}
\tikzset{
  /tikz/shadow blur radius/.store in=\pgfbs@radius,
  /tikz/shadow blur radius=.4ex,
  /tikz/shadow blur extra rounding/.store in=\pgfbs@extra@rounding,
  /tikz/shadow blur extra rounding=\pgfutil@empty,
  /tikz/shadow blur extra rounding/.default=\pgfbs@radius,
  /tikz/shadow blur steps/.store in=\pgfbs@steps,
  /tikz/shadow blur steps=4,
  /tikz/shadow opacity/.store in=\pgfbs@opacity,
  /tikz/shadow opacity=40,
  /tikz/blur shadow/.style={
    shadow scale=1,
    shadow xshift=.5ex,
    shadow yshift=-.5ex,
    preaction=render blur shadow,
    every shadow,
    #1,
  },
  /tikz/render blur shadow/.code={
    \pgfbs@savebb
    \pgfsyssoftpath@getcurrentpath{\pgfbs@input@path}%
    \pgfbs@compute@shadow@bbox
    \pgfbs@process@rounding{\pgfbs@input@path}{\pgfbs@fadepath}%
    \pgfbs@apply@canvas@transform
    \colorlet{pstb@shadow@color}{white!\pgfbs@opacity!black}%
    \pgfdeclarefading{shadowfading}{\pgfbs@paint@fading}%
    \pgfsetfillcolor{black}%
    \pgfsetfading{shadowfading}%
       {\pgftransformshift{\pgfpoint{\pgfbs@midx}{\pgfbs@midy}}}%
    \pgfbs@usebbox{fill}%
    \pgfbs@restorebb
  },
}
\def\pgfbs@savebb{%
  \edef\pgfbs@restorebb{%
    \global\pgf@picminx=\the\pgf@picminx\relax
    \global\pgf@picmaxx=\the\pgf@picmaxx\relax
    \global\pgf@picminy=\the\pgf@picminy\relax
    \global\pgf@picmaxy=\the\pgf@picmaxy\relax
  }%
}
\def\restorebb{}%
\def\pgfbs@process@rounding#1#2{
  \expandafter\ifx\pgfbs@extra@rounding\pgfutil@empty%
    \pgfprocessround{#1}{#2}%
  \else%
    \pgfmathsetmacro\pgfbs@exrd@val{\pgfbs@extra@rounding}%
    \pgfbs@roundpath{#1}{\pgfbs@exrd@val pt}%
    \pgfsyssoftpath@getcurrentpath{\pgfbs@extraroundedpath}%
    \pgfprocessround{\pgfbs@extraroundedpath}{#2}%
  \fi%
}
\def\pgfbs@roundpath#1#2{%
  {%
    \def\pgfbs@rp@skipround{%
      \let\pgfbs@rp@possibleround\pgfbs@rp@insertround}%
    \def\pgfbs@rp@insertround{\pgfsyssoftpath@specialround{#2}{#2}}%
    \let\pgfbs@rp@possibleround\pgfbs@rp@insertround%
    %
    \def\pgfsyssoftpath@movetotoken##1##2{%
      \pgfsyssoftpath@moveto{##1}{##2}}%
    \def\pgfsyssoftpath@linetotoken##1##2{%
      \pgfbs@rp@possibleround\pgfsyssoftpath@lineto{##1}{##2}}%
    \def\pgfsyssoftpath@rectcornertoken##1##2##3##4##5{%
      \pgf@xa=##1\relax%
      \advance\pgf@xa by##4%
      \pgf@ya=##2\relax%
      \advance\pgf@ya by##5%
      \pgfsyssoftpath@moveto{##1}{##2}%
      \pgfbs@rp@possibleround%
      \pgfsyssoftpath@lineto{\the\pgf@xa}{##2}%
      \pgfbs@rp@possibleround%
      \pgfsyssoftpath@lineto{\the\pgf@xa}{\the\pgf@ya}%
      \pgfbs@rp@possibleround%
      \pgfsyssoftpath@lineto{##1}{\the\pgf@ya}%
      \pgfbs@rp@possibleround%
      \pgfsyssoftpath@closepath}%
    \def\pgfsyssoftpath@curvetosupportatoken%
       ##1##2##3##4##5##6##7##8{%
      \pgfbs@rp@possibleround%
      \pgfsyssoftpath@curveto{##1}{##2}{##4}{##5}{##7}{##8}}%
    \def\pgfsyssoftpath@closepathtoken##1##2{%
      \pgfbs@rp@possibleround\pgfsyssoftpath@closepath}%
    \def\pgfsyssoftpath@specialroundtoken##1##2{%
      \pgfmathsetmacro\pgfbs@rp@ra{max(##1,#2)}%
      \pgfmathsetmacro\pgfbs@rp@rb{max(##2,#2)}%
      \pgfsyssoftpath@specialround%
          {\pgfbs@rp@ra pt}{\pgfbs@rp@rb pt}%
      \let\pgfbs@rp@possibleround\pgfbs@rp@skipround%
    }
    #1%
  }
}
\def\pgfbs@compute@shadow@bbox{%
  \edef\pgfbs@minx{\the\pgf@pathminx}%
  \edef\pgfbs@miny{\the\pgf@pathminy}%
  \edef\pgfbs@maxx{\the\pgf@pathmaxx}%
  \edef\pgfbs@maxy{\the\pgf@pathmaxy}%
  \pgfmathsetmacro\pgfbs@midx{0.5*(\pgfbs@minx + \pgfbs@maxx)}%
  \pgfmathsetmacro\pgfbs@midy{0.5*(\pgfbs@miny + \pgfbs@maxy)}%
  \pgfmathsetmacro\pgfbs@minx{\pgfbs@minx - \pgfbs@radius}%
  \pgfmathsetmacro\pgfbs@miny{\pgfbs@miny - \pgfbs@radius}%
  \pgfmathsetmacro\pgfbs@maxx{\pgfbs@maxx + \pgfbs@radius}%
  \pgfmathsetmacro\pgfbs@maxy{\pgfbs@maxy + \pgfbs@radius}%
  \pgfmathsetmacro\pgfbs@wd{\pgfbs@maxx - \pgfbs@minx}%
  \pgfmathsetmacro\pgfbs@ht{\pgfbs@maxy - \pgfbs@miny}%
  \pgfsyssoftpath@setcurrentpath\pgfutil@empty%
  \pgfsyssoftpath@rect{\pgfbs@minx pt}{\pgfbs@miny pt}%
                      {\pgfbs@wd pt}{\pgfbs@ht pt}%
  \pgfsyssoftpath@getcurrentpath{\pgfbs@shadow@bbox}%
  \pgfsyssoftpath@setcurrentpath\pgfutil@empty%
}

\def\pgfbs@set@fading@pic@bbox{
  \global\pgf@picminx=\pgfbs@minx pt\relax
  \global\pgf@picminy=\pgfbs@miny pt\relax
  \global\pgf@picmaxx=\pgfbs@maxx pt\relax
  \global\pgf@picmaxy=\pgfbs@maxy pt\relax
}
\def\pgfbs@usefadepath#1{%
  \pgfsyssoftpath@setcurrentpath{\pgfbs@fadepath}%
  \pgfsyssoftpath@flushcurrentpath%
  \pgfusepath{#1}%
}
\def\pgfbs@usebbox#1{%
  \pgfsyssoftpath@setcurrentpath{\pgfbs@shadow@bbox}%
  \pgfsyssoftpath@flushcurrentpath%
  \pgfusepath{#1}%
}
\def\pgfbs@apply@canvas@transform{
  \pgflowlevel{
    \pgftransformshift{\pgfpoint{\pgfbs@midx}{\pgfbs@midy}}
    \pgftransformscale{\pgfkeysvalueof{/tikz/shadow scale}}
    \pgftransformshift{\pgfpoint%
      {\pgfkeysvalueof{/tikz/shadow xshift}-\pgfbs@midx}
      {\pgfkeysvalueof{/tikz/shadow yshift}-\pgfbs@midy}
    }
  }
}
\def\pgfbs@paint@fading{
  \pgfpicture
    % fix bounding box.
    \pgfbs@set@fading@pic@bbox
    % compute increments for line width and opacity
    \pgfmathsetmacro\pgfbs@op@step{50/\pgfbs@steps}
    \pgfmathsetmacro\pgfbs@wth@step{4*\pgfbs@radius/(2*\pgfbs@steps-1)}
    % draw the outer part of the fading,
    % starting with lightest, outermost line
    \pgfsetroundjoin
    \pgfmathsetmacro\pgfbs@max@i{\pgfbs@steps-2}
    \pgfmathsetmacro\pgfbs@wth{2*\pgfbs@radius}
    \pgfmathsetmacro\pgfbs@op{100-0.5*\pgfbs@op@step}
    \foreach \pgfbs@i in {0,...,\pgfbs@max@i} {
      \pgfsetlinewidth{\pgfbs@wth pt}
      \pgfsetstrokecolor{black!\pgfbs@op!pstb@shadow@color}
      \pgfbs@usefadepath{stroke}
      \pgfmathsetmacro\pgfbs@wth{\pgfbs@wth-\pgfbs@wth@step}
      \global\let\pgfbs@wth=\pgfbs@wth
      \pgfmathsetmacro\pgfbs@op{\pgfbs@op-\pgfbs@op@step}
      \global\let\pgfbs@op=\pgfbs@op
    }
    % clip to inside of path
    \scope
    \pgfbs@usefadepath{clip}
    % fill inside with final darkest shadow color
    \pgfsetfillcolor{pstb@shadow@color}
    \pgfbs@usebbox{fill}
    % draw the inner part of the fading,
    % starting with the darkest, innermost line
    \pgfmathsetmacro\pgfbs@wth{2*\pgfbs@radius}
    \pgfmathsetmacro\pgfbs@op{0.5*\pgfbs@op@step}
    \foreach \pgfbs@i in {0,...,\pgfbs@max@i} {
      \pgfsetlinewidth{\pgfbs@wth pt}
      \pgfsetstrokecolor{black!\pgfbs@op!pstb@shadow@color}
      \pgfbs@usefadepath{stroke}
      \pgfmathsetmacro\pgfbs@wth{\pgfbs@wth-\pgfbs@wth@step}
      \global\let\pgfbs@wth=\pgfbs@wth
      \pgfmathsetmacro\pgfbs@op{\pgfbs@op+\pgfbs@op@step}
      \global\let\pgfbs@op=\pgfbs@op
    }
    \endscope
    % a final stroke to hide clip/antialiasing artifcats
    \pgfsetstrokecolor{black!50!pstb@shadow@color}
    \pgfsetlinewidth{0.5*\pgfbs@wth@step}
    \pgfbs@usefadepath{stroke}
  \endpgfpicture
}
\endinput
%%
%% End of file `tikzlibraryshadows.blur.code.tex'.

